RAR-b: Reasoning as Retrieval Benchmark

Semantic textual similartiy (STS) and information retrieval tasks (IR) tasks have been the two major avenues to record the progress of embedding models in the past few years. Under the emerging Retrieval-augmented Generation (RAG) paradigm, we envision the need to evaluate next-level language understanding abilities of embedding models, and take a conscious look at the reasoning abilities stored in them. Addressing this, we pose the question: Can retrievers solve reasoning problems? By transforming reasoning tasks into retrieval tasks, we find that without specifically trained for reasoning-level language understanding, current state-of-the-art retriever models may still be far from being competent for playing the role of assisting LLMs, especially in reasoning-intensive tasks. Moreover, albeit trained to be aware of instructions, instruction-aware IR models are often better off without instructions in inference time for reasoning tasks, posing an overlooked retriever-LLM behavioral gap for the research community to align. However, recent decoder-based embedding models show great promise in narrowing the gap, highlighting the pathway for embedding models to achieve reasoning-level language understanding. We also show that, although current off-the-shelf re-ranker models fail on these tasks, injecting reasoning abilities into them through fine-tuning still appears easier than doing so to bi-encoders, and we are able to achieve state-of-the-art performance across all tasks by fine-tuning a reranking model. We release Reasoning as Retrieval Benchmark (RAR-b), a holistic suite of tasks and settings to evaluate the reasoning abilities stored in retriever models. RAR-b is available at https://github.com/gowitheflow-1998/RAR-b.

==> tables/L3_retrieval_all.tex <==
% \begin{table}[!htp]\centering
% \caption{L3 Full-Retrieval nDCG@10}\label{tab: L3 full all}
% \scalebox{0.9}{
% \begin{tabular}{lrccccc}\toprule
% \multicolumn{2}{c}{Model Dataset} &Math-pooled &TempReason avg. &SpartQA &Code-pooled \\\midrule
% \multirow{2}{*}{Contriever} &w/o Inst &0.579 &\textbf{0.177} &\textbf{0.149} &\ 0.061 \\
% &w/ Inst &0.524 &\textbf{0.172} &\textbf{0.159} & 0.049 \\
% \midrule
% \multirow{2}{*}{all-mpnet-base-v2} &w/o Inst &\textbf{0.899} &0.099 &0.031 & 0.148\\
% &w/ Inst &\textbf{0.898} &0.079 &0.046 & 0.122 \\
% \multirow{2}{*}{all-MiniLM-L6-v2} &w/o Inst &0.863 &0.117 &0.056 & 0.106 \\
% &w/ Inst &0.851 &0.106 &0.038 & 0.117 \\
% \multirow{2}{*}{Dragon+} &w/o Inst &0.682 &0.136 &0.116 & 0.122 \\
% &w/ Inst &0.647 &0.136 &0.122 & 0.113 \\
% \midrule
% \multirow{2}{*}{InstructOR-base} &w/o Inst &0.802 &0.091 &0.076 & 0.225\\
% &w/ Inst &0.804 &0.085 &0.113 & 0.207 \\
% \multirow{2}{*}{InstructOR-large} &w/o Inst &0.872 &0.108 &0.049 & \textbf{0.285}\\
% &w/ Inst &0.851 &0.096 &0.055 & 0.216 \\
% \multirow{2}{*}{InstructOR-XL} &w/o Inst &0.817 &0.114 &0.031 & 0.208\\
% &w/ Inst &0.819 &0.105 &0.056 & \textbf{0.247} \\
% \multirow{2}{*}{bge-small} &w/o Inst &0.738 &0.114 &0.054 & 0.183 \\
% &w/ Inst &0.765 &0.112 &0.049 & 0.199\\
% \multirow{2}{*}{bge-base} &w/o Inst &0.737 &0.113 &0.063 & 0.157\\
% &w/ Inst &0.762 &0.109 &0.050 & 0.139\\
% \multirow{2}{*}{bge-large} &w/o Inst &0.804 &0.138 &0.064 & 0.229\\
% &w/ Inst &0.797 &0.130 &0.059 & 0.215 \\
% \bottomrule
% \end{tabular}}
% \end{table}

==> tables/multiple_choice_analysis_legacy.tex <==
% %\usepackage{booktabs, multirow} % for borders and merged ranges
% %\usepackage{soul}% for underlines
% %\usepackage[table]{xcolor} % for cell colors
% %\usepackage{changepage,threeparttable} % for wide tables
% %If the table is too wide, replace \begin{table}[!htp]...\end{table} with
% %\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
% \begin{table}[!htp]\centering
% \caption{Performance Breakdown analysis in Multiple-Choice Retrieval (MCR) setting. The \textbf{upper part} of the table presents the performance gain of each model to the corresponding random baseline in relative percentage. For each model, we report the best out of its performances w/ or w/o instruction prompts. The \textbf{lower part} of the table presents the performance gains brought by instruction prompts. Surpringsly, instruction prompts lead to performance degradation for most datasets, even for models that are trained to be aware of instructions.}\label{tab: mcr analysis}
% \scriptsize
% \begin{tabular}{lcccc|c|ccc|c} \\ \toprule
% \multicolumn{1}{l}{Model $\downarrow$ \space Dataset $\rightarrow$}&$\alpha$NLI &HellaSwag &PIQA &SIQA &L1 Avg. &WinoG &CSTS-E &CSTS-H &L2 Avg. \\\midrule
% \multicolumn{2}{l}{\textit{Performance gains to baseline}} &&&&&&&&\\

% Contriever &2.74\% &23.48\% &15.02\% &16.86\% &14.53\% &0.56\% &-5.42\% &-11.86\% &-5.57\% \\
% all-mpnet-base-v2 &10.70\% &39.92\% &17.42\% &24.51\% &23.14\% &\underline{2.92\%} &\textbf{2.26\%} &-19.02\% &-4.61\% \\
% all-MiniLM-L6-v2 &0.52\% &28.80\% &14.68\% &18.24\% &15.56\% &2.60\% &-5.24\% &-9.24\% &-3.96\% \\
% Dragon & 3.14\% & 21.56\% & 17.08\% & 17.91\% & 14.92\% & \textbf{3.08\%} & -9.42\% & -12.40\% & -6.25\%\\
% InstructOR-base &11.88\% &37.76\% &22.30\% &28.20\% &25.04\% &-0.56\% &-1.74\% &-2.10\% &-1.47\% \\
% InstructOR-large &\underline{14.36\%} &\underline{53.92\%} &\underline{27.42\%} &\textbf{40.35\%} &\underline{34.01\%} &-1.50\% &-4.36\% &-3.50\% &-3.12\% \\
% InstructOR-XL &\textbf{14.88\%} &\textbf{59.20\%} &\textbf{30.90\%} &\underline{31.59\%} &\textbf{34.14\%} &2.14\% &\underline{-0.18\%} &-5.44\% &-1.16\% \\
% bge-small & 5.74\% & 30.24\% & 16.22\% & 26.07\% & 19.57\% & -0.86\% & -11.18\% & \textbf{4.18\%} & -2.62\% \\
% bge-base & 7.18\% & 34.32\% & 18.60\% & 28.35\% & 22.11\% & 2.44\% & -3.84\% & -1.74\% & \underline{-1.05\%} \\
% bge-large & 8.94\% & 40.04\% & 19.58\% & 29.58\% & 24.54\% & 0.40\% & -0.52\% & \underline{3.50\%} & \textbf{1.13\%} \\
% \midrule
% \multicolumn{2}{l}{\textit{Gains of Instruction Prompts}} &&&&&&&&\\
% Contriever &-3.06\% &\textbf{0.68\%} &-3.22\% &1.06\% &-1.13\% &0.96\% & / & / & / \\
% all-mpnet-base-v2 &-2.24\% &-9.83\% &-4.17\% &-0.60\% &-4.21\% &0.31\% & / & / & / \\
% all-MiniLM-L6-v2 &\textbf{1.31\%} &-2.17\% &-0.84\% &-0.28\% &\underline{-0.49\%} &-3.37\% & / & / & / \\
% Dragon & \underline{0.00\%} & -2.04\% & -2.22\% & -0.25\% & -1.13\% & 1.56\% & / & / & / \\
% InstructOR-base &-3.04\% &-3.05\% &-3.73\% &-4.77\% &-3.65\% &0.46\% & / & / & / \\
% InstructOR-large &-1.82\% &-6.11\% &\textbf{-0.35\%} &-5.58\% &-3.46\% &1.30\% & / & / & / \\
% InstructOR-XL &-2.61\% &-4.32\% &-2.99\% &-2.46\% &-3.10\% &\underline{1.90\%} & / & / & / \\
% bge-small & -1.36\% & -0.95\% & -2.44\% & \textbf{1.99\%} & -0.69\% & \textbf{3.64\%} & / & / & / \\
% bge-base & -0.37\% & -1.61\% & -3.31\% & 0.97\% & -1.08\% & -0.92\% & / & / & / \\
% bge-large & -0.18\% & \underline{0.34\%} & \underline{-0.82\%} & \underline{1.08\%} & \textbf{0.10\%} & -2.21\% & / & / & /\\
% \bottomrule
% \end{tabular}
% \end{table}

==> tables/multiple_choice_performance_legacy.tex <==
% %\usepackage{booktabs, multirow} % for borders and merged ranges
% %\usepackage{soul}% for underlines
% %\usepackage[table]{xcolor} % for cell colors
% %\usepackage{changepage,threeparttable} % for wide tables
% %If the table is too wide, replace \begin{table}[!htp]...\end{table} with
% %\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
% \begin{table}[!htp]\centering
% \caption{Retriever Performance in Multiple-Choice Retrieval (MCR) setting. Random baseline is computed by available choices in each dataset. We present the performance with and without instruction prompts for each model. Notably, due to the OOD task nature of CSTS, it makes less sense to include the w/o instruction setting, as we carefully craft the retrieval tasks that are not meaningful to retrieve without a clear stated purpose (which must be realized by an instruction prompt).}\label{tab: mcr table}
% % \scriptsize
% \scalebox{0.9}{%
% \begin{tabular}{lrccccccc}\\ \toprule
% \multicolumn{2}{l}{Model $\downarrow$ \quad Dataset $\rightarrow$} &$\alpha$NLI &HellaSwag &PIQA &SIQA &WinoG &CSTS-E &CSTS-H \\\midrule
% Random Baseline &\multicolumn{1}{c}{/} &50.00 &25.00 &50.00 &33.33 &50.00 &50.00/50.00 &50.00 \\
% \midrule
% \multirow{2}{*}{Contriever} &w/o Inst. &51.37 &30.66 &57.51 &38.54 &49.80 & & \\
% &w/ Inst. &49.80 &30.87 &55.66 &38.95 &50.28 &47.29/44.94 &44.07 \\
% \midrule
% \multirow{2}{*}{all-mpnet-base-v2} &w/o Inst. &55.35 &34.98 &58.71 &41.50 &51.30 & & \\
% &w/ Inst. &54.11 &31.54 &56.26 &41.25 &51.46 &49.65/51.13 &40.49 \\
% \multirow{2}{*}{all-MiniLM-L6-v2} &w/o Inst. &49.61 &32.20 &57.34 &39.41 &51.30 & & \\
% &w/ Inst. &50.26 &31.50 &56.86 &39.30 &49.57 &47.38/45.29 &45.38 \\
% \multirow{2}{*}{Dragon} & w/o Inst. & 51.57 & 30.39 & 58.54 & 39.30 & 50.75 & & \\
% & w/ Inst. & 51.57 & 29.77 & 57.24 & 39.20 & 51.54 & 45.29/44.76 & 43.8 \\
% \midrule
% \multirow{2}{*}{InstructOR-base} &w/o Inst. &55.94 &34.44 &61.15 &42.73 &49.49 & & \\
% &w/ Inst. &54.24 &33.39 &58.87 &40.69 &49.72 &46.77/49.13 &48.95 \\
% \multirow{2}{*}{InstructOR-large} &w/o Inst. &57.18 &38.48 &63.71 &46.78 &48.62 & & \\
% &w/ Inst. &56.14 &36.13 &63.49 &44.17 &49.25 &44.07/47.82 &48.25 \\
% \multirow{2}{*}{InstructOR-XL} &w/o Inst. &57.44 &39.80 &65.45 &43.86 &50.12 & & \\
% &w/ Inst. &55.94 &38.08 &63.49 &42.78 &51.07 &45.20/49.91 &47.28 \\
% \multirow{2}{*}{bge-small} & w/o Inst. & 52.87 & 32.56 & 58.11 & 41.20 & 47.83 & & \\
% & w/ Inst. & 52.15 & 32.25 & 56.69 & 42.02 & 49.57 & 44.41/42.23 & 52.09 \\
% \multirow{2}{*}{bge-base} & w/o Inst. & 53.59 & 33.58 & 59.30 & 42.37 & 51.22 & & \\
% & w/ Inst. & 53.39 & 33.04 & 57.34 & 42.78 & 50.75 & 48.08/45.90 & 49.13 \\
% \multirow{2}{*}{bge-large} & w/o Inst. & 54.47 & 34.89 & 59.79 & 42.73 & 50.20 & & \\
% & w/ Inst. & 54.37 & 35.01 & 59.30 & 43.19 & 49.09 & 49.30/49.74 & 51.75 \\

% \bottomrule
% \end{tabular}}
% \end{table}
